J-P: MDP. FP. PP.: Characterizing Total Expected Rewards in Markov Decision Processes as Least Fixed Points with an Application to Operational Semantics of Probabilistic Programs (Technical Report)

Markov decision processes (MDPs) with rewards are a widespread and well-studied model for systems that make both probabilistic and nondeterministic choices. A fundamental result about MDPs is that their minimal and maximal expected rewards satisfy Bellmann's optimality equations. For various classes of MDPs - notably finite-state MDPs, positive bounded models, and negative models - expected rewards are known to be the least solution of those equations. However, these classes of MDPs are too restrictive for probabilistic program verification. In particular, they assume that all rewards are finite. This is already not the case for the expected runtime of a simple probabilisitic program modeling a 1-dimensional random walk. In this paper, we develop a generalized least fixed point characterization of expected rewards in MDPs without those restrictions. Furthermore, we demonstrate how said characterization can be leveraged to prove weakest-preexpectation-style calculi sound with respect to an operational MDP model.

==> some_introtext.tex <==
We consider countably infinite-state Markov decision processes (MDPs) and undiscounted expected rewards for $\PosRealsInf$-valued reward functions. MDPs are a suitable model for an operational semantics of probabilistic programs (cf.\ \Cref{sec:prelim:pgcl:opsem}). The notion of expected rewards enables us to establish a connection between this operational semantics and the deductive verification techniques employed in this paper (cf.\ \Cref{sec:prelim:wp:wp_vs_op}).

We rely on least fixpoint characterizations of minimal and maximal expected rewards in MDPs, i.e., on the fact that expected rewards are given as the least solution of Bellman's optimality equations \cite{Bellman1957MDPs}. These least fixpoint characterizations are well-understood in various settings (see, e.g., \cite[Theorem 7.2.3a and Theorem 7.3.3a]{puterman}). There is, however, a slight mismatch between the notion of expected rewards considered in the literature and the notion required in this paper: For \emph{maximal} expected rewards, our setting is closely related to what \cite[Section 7.2]{puterman} calls \emph{positive bounded models}. \cite[Section 7.2]{puterman} assumes that both reward functions and corresponding maximal expected rewards are \emph{pointwise smaller than $\infty$} (cf.\ \cite[Assumption 7.2.1]{puterman}). We cannot rely on this assumption since $\infty$-valued maximal expected rewards occur naturally when reasoning about expected outcomes of probabilistic programs (cf.\ \Cref{rem:prelim:wp:infty}). Similarly, for  \emph{minimal} expected rewards, our setting is closely related to what \cite[Section 7.3]{puterman} calls \emph{negative models}. Even though $\infty$-valued minimal expected rewards are not excluded, reward functions are assumed to be pointwise smaller than $\infty$ --- another assumption we cannot rely on.

For this reason, we employ the concepts from domain theory presented in \Cref{sec:prelim:domain_theory} to derive least fixpoint characterizations of possibly $\infty$-valued minimal and maximal expected rewards and prove these characterizations correct. We proceed as follows: In \Cref{sec:mdp:def}, we define MDPs alongside corresponding basic notions such as paths and schedulers. In \Cref{sec:mdp:exprew}, we introduce the notion of expected rewards in MDPs considered in this paper and study their properties in \Cref{sec:mdp:exprewprop}. The least fixpoint characterizations of expected rewards are treated in \Cref{sec:mdp:exprew_lfp}. We then conclude with a note on the existence of \emph{optimal} schedulers in \Cref{sec:mdp:strategies}.
